Transmission Investment Coordination using MILP Lagrange Dual Decomposition and Auxiliary Problem Principle

This paper considers the investment coordination problem for the long term transmission capacity expansion in a situation where there are multiple regional Transmission Planners (TPs), each acting in order to maximize the utility in only its own region. In such a setting, any particular TP does not normally have any incentive to cooperate with the neighboring TP(s), although the optimal investment decision of each TP is contingent upon those of the neighboring TPs. A game-theoretic interaction among the TPs does not necessarily lead to this overall social optimum. We, therefore, introduce a social planner and call it the Transmission Planning Coordinator (TPC) whose goal is to attain the optimal possible social welfare for the bigger geographical region. In order to achieve this goal, this paper introduces a new incentive mechanism, based on distributed optimization theory. This incentive mechanism can be viewed as a set of rules of the transmission expansion investment coordination game, set by the social planner TPC, such that, even if the individual TPs act selfishly, it will still lead to the TPC's goal of attaining overall social optimum. Finally, the effectiveness of our approach is demonstrated through several simulation studies.

==> VCG.tex <==
In this section, we will consider a variant of our proposed mechanism design in order to induce a truth-telling behavior about the decision to build or, not to build lines by the respective zones. 

==> multipleStepSimultaneous.tex <==
In this section, we will allow for the capacity expansion for generation and transmission to happen in multiple discrete steps, while still assuming that the generators and transmission lines make simultaneous moves. Hence, we introduce the integer binary decision variables $x$s into the optimization formulations. The angles included version is as follows:\\
%----------------------------------------------------------------------------------------------------------------------------------------
\begin{subequations}\label{Step2:General}
\begin{gather}
\min_{P_{g_q}}\sum_{g_q\in{G}}[C_{g_q}(P_{g_q})+C_{g_q}({\hat{P_{g_q}}})]+\sum_{T_r\in{T}}C_{T_r}({\hat{L}}_{T_r})\label{first_Step2:General}\\
\mbox{Subject\;to:\:}P_{{g_q}_{N_i}}-P_{{D_d}_{N_i}}=\sum_{N_{\overline{i}}\in{J(N_i)}}B_{T_r}(\theta_{N_i}-\theta_{N_{\overline{i}}})\notag\\ \forall{{N_i}\in\mathcal{N}}\label{second_Step2:General}\\
|B_{T_r}(\theta_{{T_r}_{t_1}}-\theta_{{T_r}_{t_2}})|\leq{{\overline{L}}_{T_r}+{\hat{L}}_{T_r}},\;\forall{T_r\in{T}}\notag\\\label{third_Step2:General}
{\underline{P}}_{g_q}\leq P_{g_q}\leq{{\overline{P}}_{g_q}+{\hat{P}}_{g_q}},\;\forall{g_q\in{G}}\label{fourth_Step2:General}\\
x^{\omega}_{T_r}\in\{0,1\},\;\forall{T_r\in{T}},\;x{\omega}_{g_q}\in\{0,1\},\;\forall{g_q\in{G}},\;\label{fifth_Step2:General}\\
{\hat{L}}_{T_r}=\sum_{\omega}A_{\omega}x^{\omega}_{T_r}{\hat{L}}^{max}_{T_r},\;\forall{T_r\in{T}}\label{sixth_Step2:General}\\
{\hat{P}}_{g_q}=\sum_{\omega}A_{\omega}x^{\omega}_{g_q}{\hat{P}}^{max}_{g_q},\;\forall{g_q\in{G}},\;\label{seventh_Step2:General}
\end{gather}
\end{subequations}
%----------------------------------------------------------------------------------------------------------------------------------------
As before, $J(N_i)$ is the set of all the buses that are directly connected to bus $N_i$. $B_{T_r}$ is the series susceptance of the transmission line whose terminals are either indicated explicitly as subscripts of the voltage angles in the multiplier or are implicit in the node indices of the same.
The alternative formulation with the angles eliminated is as follows:
%----------------------------------------------------------------------------------------------------------------------------------------
\begin{subequations}\label{Step1:General_Alternative}
\begin{gather}
\min_{P_{g_q}}\sum_{g_q\in{G}}[C_{g_q}(P_{g_q})+C_{g_q}({\hat{P_{g_q}}})]+\sum_{T_r\in{T}}C_{T_r}({\hat{L}}_{T_r})\label{first_Step1:General_Alternative}\\
\mbox{Subject\;to:\:}\sum_{g_q\in G}P_{g_q}=\sum_{D_d\in L}P_{D_d}\label{second_Step1:General_Alternative}\\
|\Phi{(\mathbf{P_g}-\mathbf{P_D})}|\leq{\mathbf{\overline{L}}}+{\mathbf{\hat{L}}}\label{third_Step1:General_Alternative}\\
{\underline{P}}_{g_q}\leq P_{g_q}\leq{{\overline{P}}_{g_q}+x_{g_q}{\hat{P}}_{g_q}},\;\forall{g_q\in{G}}\label{fourth_Step2:General_Alternative}\\
x^{\omega}_{T_r}\in\{0,1\},\;\forall{T_r\in{T}},\;x^{\omega}_{g_q}\in\{0,1\},\;\forall{g_q\in{G}},\;\label{fifth_Step2:General_Alternative}\\
{\hat{L}}_{T_r}=\sum_{\omega}A_{\omega}x^{\omega}_{T_r}{\hat{L}}^{max}_{T_r},\;\forall{T_r\in{T}}\label{sixth_Step2:General_Alternative}\\
{\hat{P}}_{g_q}=\sum_{\omega}A_{\omega}x^{\omega}_{g_q}{\hat{P}}^{max}_{g_q},\;\forall{g_q\in{G}},\;\label{sixth_Step2:General_Alternative}
\end{gather}
\end{subequations}
%----------------------------------------------------------------------------------------------------------------------------------------
where the symbols that has been re-used has the same meanings, as in the previous section.
